Extractive Schema Linking for Text-to-SQL

Text-to-SQL is emerging as a practical interface for real world databases. The dominant paradigm for Text-to-SQL is cross-database or schema-independent, supporting application schemas unseen during training. The schema of a database defines the tables, columns, column types and foreign key connections between tables. Real world schemas can be large, containing hundreds of columns, but for any particular query only a small fraction will be relevant. Placing the entire schema in the prompt for an LLM can be impossible for models with smaller token windows and expensive even when the context window is large enough to allow it. Even apart from computational considerations, the accuracy of the model can be improved by focusing the SQL generation on only the relevant portion of the database. Schema linking identifies the portion of the database schema useful for the question. Previous work on schema linking has used graph neural networks, generative LLMs, and cross encoder classifiers. We introduce a new approach to adapt decoder-only LLMs to schema linking that is both computationally more efficient and more accurate than the generative approach. Additionally our extractive approach permits fine-grained control over the precision-recall trade-off for schema linking.

==> schema_link_example.tex <==
\begin{figure}
    \centering
\begin{quote}\begin{small}
CREATE TABLE publication (\\
 publication\_id NUMBER PRIMARY KEY,\\
 book\_id NUMBER,\\
 publisher TEXT,\\
 publication\_date TEXT,\\
 price NUMBER,\\
 FOREIGN KEY(book\_id) REFERENCES book(book\_id)
);\\
[\baselineskip]
CREATE TABLE book (\\
 book\_id NUMBER PRIMARY KEY,\\
 title TEXT,\\
 issues NUMBER,\\
 writer TEXT
);\\
[\baselineskip]
To answer:
Show the titles of books in descending order of publication price.\\
We need columns:\\
« publication publication\_id»\\
« publication book\_id»\\
« publication publisher»\\
« publication publication\_date»\\
« publication price»\\
« book book\_id»\\
« book title»\\
« book issues»\\
« book writer»\\
\end{small}\end{quote}
    \caption{Example schema linker input}
    \label{fig:schema_link_input}
\end{figure}

\begin{figure}
    \centering
\begin{quote}\begin{small}
CREATE TABLE publication (\\
 book\_id NUMBER,\\
 price NUMBER,\\
 FOREIGN KEY(book\_id) REFERENCES book(book\_id)
);\\
[\baselineskip]
CREATE TABLE book (\\
 book\_id NUMBER PRIMARY KEY,\\
 title TEXT,
);\\
[\baselineskip]
Show the titles of books in descending order of publication price.\\
\end{small}\end{quote}
    \caption{Focused schema input}
    \label{fig:focused_schema_input}
\end{figure}


\begin{figure}
    \centering
\begin{quote}\begin{small}
CREATE TABLE singer (\\
 singer\_id NUMBER PRIMARY KEY,\\
 name TEXT,\\
 birth\_year NUMBER,\\
 net\_worth\_millions NUMBER,\\
 citizenship TEXT
);\\
[\baselineskip]
CREATE TABLE song (\\
 song\_id NUMBER PRIMARY KEY,\\
 title TEXT,\\
 singer\_id NUMBER,\\
 sales NUMBER,\\
 highest\_position NUMBER,\\
 FOREIGN KEY(singer\_id) REFERENCES singer(singer\_id)
);\\
[\baselineskip]
To answer:
How many singers are there?\\
We need columns:\\
« singer singer\_id»\\
« singer name»\\
« singer birth\_year»\\
« singer net\_worth\_millions»\\
« singer citizenship»\\
« song song\_id»\\
« song title»\\
« song singer\_id»\\
« song sales»\\
« song highest\_position»\\
\end{small}\end{quote}
    \caption{The shortest schema linking example from the Spider train set.}
    \label{fig:schema_link_input}
\end{figure}
